Novel Matrix Hit and Run for Sampling Polytopes and Its GPU Implementation

We propose and analyze a new Markov Chain Monte Carlo algorithm that generates a uniform sample over full and non-full dimensional polytopes. This algorithm, termed "Matrix Hit and Run" (MHAR), is a modification of the Hit and Run framework. For the regime $n^{1+\frac{1}{3}} \ll m$, MHAR has a lower asymptotic cost per sample in terms of soft-O notation ($\SO$) than do existing sampling algorithms after a \textit{warm start}. MHAR is designed to take advantage of matrix multiplication routines that require less computational and memory resources. Our tests show this implementation to be substantially faster than the \textit{hitandrun} R package, especially for higher dimensions. Finally, we provide a python library based on Pytorch and a Colab notebook with the implementation ready for deployment in architectures with GPU or just CPU.

==> cambios.tex <==
Cambie el abstract
\begin{abstract}
We propose and analyze a new Markov Chain Monte Carlo algorithm that generates a uniform sample over full and non-full dimensional polytopes. We named this algorithm "Matrix Hit and Run" (MHAR) since it is a modified version of the well-known Hit and Run framework. Depending on the dimension and number of restrictions, the MHAR has the lowest asymptotic \textit{cost per sample} compared to state of the art algorithms. We present an implementation of the MHAR that takes advantage of matrix multiplication routines designed for GGPUs and CPUs that are efficient in terms of operations and memory management, and provide a set of experimental results to test its efficiency. The implementation shows substantial speedups in comparison to the \textit{hitandrun} R package specially in higher dimensions. Finally, we provide a python library based on Pytorch and a Colab notebook with the implementation ready for deployment in GPU-CPU architectures. 
\end{abstract}

Pase a no comentarios los pies de paginas de las tablas



El inicio de la seccion de experimentos donde hablo de pytorch, y agregue su cita a la bibliografia:

\subsection{Code}
We coded the MHAR using python and the Pytorch library. This allowed us to use a high level language and avoid any manual thread control. During all of our experiments, we never experienced any problems due to numerical instability. The maximum error we found for the inversion matrix was of the order $1e-16$ which we think is robust enough for most applications. Furthermore, almost all operations are carried out in the GPU from matrix inversion, random number generation, matrix-to-matrix multiplication and point wise operations. The only operations that need to be carried out outside the CPU are reading the constraints and saving the samples to disk, any arithmetic operation and random number is done directly in GPU.\\

Due to the structure of our code we can safely say that the overall performance depends of the GPU available and the connection speed between host-device. Note that given the flexibility of the Pytorch framework the code also works in CPU (no GPU is needed), but given the nature of the problem and the high dimensions we aim to sample we decided to focus our analysis to experiments that make use of the GPU.\\
The decision to use Pytorch as backend responds to its flexibily, power and popularity \cite{paszke2019pytorch}.





lemma 4.3











7/8/20

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Modifique el parrafo de abajo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Second, we show that the \textit{cost per sample} of the MHAR depends entirely on $m, n, z$ and $\omega$, where $m, n$ are as described in the definition of $\Delta$, $\omega$ represents a matrix multiplication coefficient as described in Table \ref{table:1}, and $z$ is a padding hyper-parameter specified by the user. After proper pre-processing and a \textit{warm start} the algorithm has a \textit{cost per sample} of $\SO\big(\min(m_I^{\omega -2}n^4, m_In^{\omega +1})\big)$ for the full dimensional scenario, and of $\SO\big(\min(n^{\omega +2}, m_In^{\omega +1})\big)$ for the non-full dimensional one.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Modifique el parrafo de abajo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For clarity and simplicity, we will refer to HAR as the algorithm presented in \cite{montiel_jd}, which extends \cite{firs_har_ever} for non-full dimensional polytopes. In addition, to ease comparison we make use of "soft-O" notation $\SO$, which suppresses $log(n)$ factors and other parameters like error bounds since it is a common practice in this area, see \cite{walks}, \cite{original-har}, and \cite{RHMC}. In the case of the HAR and the MHAR after proper pre-processing and from a \textit{warm start} the  \textit{mixing time} is of the non-deterministic order $\SO(n^3)$ as showed in \cite{original-har}. We also use $f \ll g$ notation to define a relation where $f\in \OO(g)$. Hence, if $A$ and $B$ are two algorithms, we use  $A \ll B$ to explain that the overall upper bound complexity of $B$ bounds the overall upper bound complexity of $A$, in other words $A$ is as efficient as $B$ in terms of complexity.  Finally, we assume the existence of a random stream of bits that allow us to generate a random number in $\OO(1)$.








The HAR sampling method can be described as follows. A \textit{walk} is initialized in a strict inner point of the polytope. At any iteration, a random direction is generated via independent normal variates. The random direction, along with the current point, generates a line set $L$, and its intersection with the polytope generates a line segment. The sampler selects a random point that lives in $L$ and repeats the process. The HAR algorithm for full-dimensional convex bodies, after \textit{warm start}, has a \textit{cost per sample} of $\SO(m_I n^4)$ \cite{walks}, which is a special case of Theorem \ref{th_cost_per_sample_har_nf} that states that in general the \textit{cost per sample} of the HAR is $\SO(n^3\max\{ m_In,m_E^{\omega-2}n^2\})$ after proper pre-processing and a \textit{warm start}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Agregue los siguientes dos parrafos y modifique el de arriba%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In general, the non-deterministic \textit{mixing time} of the HAR is of order $\SO(n^2 \gamma_{\kappa})$, where $ \gamma_{\kappa}$ is defined:
\[ 
 \gamma_{\kappa} = \inf_{R_{in}, R_{out}>0}\{ \frac{R_{in}}{R_{out}} \| \mathcal{B}(x, R_{in}) \subseteq \Delta \subseteq \mathcal{B}(y, R_{out}) \ for \ some \ x,y \in \Delta\}
\]
Where $R_{in}$ and $R_{out}$ are the radius of an inscribed and circumscribed ball of the polytope $\Delta$, and $\mathcal{B(q,R)}$ is the ball of radius $R$ with containing the point q. In essence
$ \gamma_{\kappa}$ is the coefficient generated by the biggest inscribed ball and the smallest circumscribed ball of the polytope. Intuitively the fact that the \textit{mixing time} depends on this parameters means that elongated polytopes are harder to sample. It is a common practice in literature to analyze the HAR algorithms for convex bodies after some pre-processing and invoking a \textit{warm start} , meaning that the body in question is brought to a near isotropic position in $\SO(\sqrt{n})$ allowing us to express the \textit{mixing time} as $\SO(n^3)$ see \cite{walks}, \cite{geo-walk}, \cite{RHMC}, \cite{ballwalk}, \cite{original-har} and \cite{har_tommi}. In order to retain comparability between literature we assume that the polytope has received proper pre-processing for the remainder of the paper.


Modifique substancialmente la seccion  5 y 6


agregue conclusiones

cambie teorema 4.10 (importante del mhar), y 3.3 (importante del har)

agregue el anexo
